Optimal Partition of a Tree with Social Distance

We study the problem to find a partition of \textcolor{black}{a} graph $G$ with maximum social welfare based on social distance between vertices in $G$, called MaxSWP. This problem is known to be NP-hard in general. In this paper, we first give a complete characterization of optimal partitions of trees with small diameters. Then, by utilizing these results, we show that MaxSWP can be solved in linear time for trees. Moreover, we show that MaxSWP is NP-hard even for 4-regular graphs.

==> conclusion.tex <==
%!TEX root = template.tex
\section{Conclusion}\label{sec:conc}
%本論文では, 木の最適社会効用分割がどのような構造をとるかを調べるとともに, これを発見するアルゴリズムを設計した. 
In this paper, we examined the structure of optimal social welfare partition of trees and designed an algorithm to find optimal solution in trees.
%まず木の部分クラスであるパスグラフについては, 最適分割の完全な特徴づけを与えた. 
For path graphs which are subclass of trees, we gave complete characterization of optimal partition.
%一般の木に対しては, 直径が小さい木の形をとる提携の社会効用値の上界値を見積もることにより, 任意の木の最適分割においては各提携が直径3以下の部分木の形をとることを示した. 
For general trees, by estimating the upper bound for the social welfare, we showed that each coalition has the diameter is three or less in optimal partition of a tree.
%この性質を利用することにより, 動的計画法に基づく木の最適分割を求めるアルゴリズムを設計した. このアルゴリズムの計算量は$O(\Delta^2n)$時間である. 
By using this property, we designed an algorithm for finding optimal partition of trees based on dynamic programming method. The computational complexity of this algorithm is $O(\Delta^2n)$ time.

%最適分割を構成する提携の形が定数個に限定され, かつ動的計画法を適用できるようなグラフクラスであれば, 同様の多項式時間アルゴリズムの設計が期待できる. 
A similar polynomial time algorithm can be expected as long as it is a graph class that is limited to a constant number of coalition constituting the optimal partition and to which dynamic programming can be applied.
%本論文により, 木の最適分割が多項式時間で求まることが明らかになったが, 木の上位クラスで同様の結果が得られるかどうかは不明である. 
In this paper, it became clear that the optimal partition of trees can be obtained with polynomial time, but it is unknown whether similar results can be obtained in the superior class of trees.
%一方, 現在知られているNP困難性は次数制限のあるグラフに留まっており, グラフの構造的な特徴との関係についてもわかっていないことが多い. 
On the other hand, the currently known NP difficulty is limited to graphs with degree restrictions, and the relationship with the structural features of the graph is often unknown in many cases.
%以上から, NP困難性と多項式時間可解の境界をグラフクラスの観点から解明することが今後の課題として挙げられる. 
From the above, it is a future task to clarify the boundary between NP difficulty and polynomial time solvable from the viewpoint of graph class.

==> relatedwork.tex <==
%!TEX root = template.tex
\section{Related work}\label{sec:relate}
Partition with social distance has been resarched as social distances games (SDGs) in coalition forming games \cite{Branzei2011}.
Coalition forming game is one of the coalition structure forming problem which is natural abstraction of one of the most important challenges in multi-agent systems. If you know the coalition structure forming problem more, please read this survey \cite{RAHWAN2015139}.

On the other hand, there are researches where they divide with quality function to partition.
In recent years, researches on modularity proposed by Newman et al. \cite{PhysRevE.69.026113} are particularly popular.
Variability approximation algorithms have been proposed since the NP-hard was shown in 2008 \cite{Brandes:980374}.
Please see this paper for details \cite{Fortunato2010}.

The former performs division under the action of the agent actively.
The latter does not impose such a condition, it divides under the evaluation basis.
Our research follows the former condition as mentioned earlier.

In coalition forming games, there are many researches about partition based on various utilities has been studied.
For example, In \cite{SLESS2018217}, each agent's utility is her sum value of the members of coalition, where value is given integer.
Moreover, There are researches with utility that is her average value of the members of coalition \cite{AzizBBHOP17}.
They are subclass of hedonic games (HGs) which have been considered with various stability concepts \cite{Dreze1980,BOGOMOLNAIA2002201,Elkind:2009}.
Similarly, in SDGs, the various fundamental notions of stability such as core stability \cite{Branzei2011}, Nash stability \cite{Balliu2017a} and Pareto stability \cite{Balliu2017b} have been already investigated.
For any stable concepts, it is important that the ratio between stable solution and maximum solution (ie., Price of Anarchy \cite{Koutsoupias1999}, Price of Pareto Optimality \cite{ElkindFF16}).

Unfortunately, about maximum solution, little is known except that it is NP-hard in the graph of maximum degree $6$ \cite{Balliu2017b} and that the approximate solution is $1/2$ or more \cite{Branzei2011}.
In spite of that approximate solution is found by using a tree, we do not know whether there is a polynomial time algorithm for finding the maximum solution in a tree.

